Image-to-Image Regression with Distribution-Free Uncertainty Quantification and Applications in Imaging

Image-to-image regression is an important learning task, used frequently in biological imaging. Current algorithms, however, do not generally offer statistical guarantees that protect against a model's mistakes and hallucinations. To address this, we develop uncertainty quantification techniques with rigorous statistical guarantees for image-to-image regression problems. In particular, we show how to derive uncertainty intervals around each pixel that are guaranteed to contain the true value with a user-specified confidence probability. Our methods work in conjunction with any base machine learning model, such as a neural network, and endow it with formal mathematical guarantees -- regardless of the true unknown data distribution or choice of model. Furthermore, they are simple to implement and computationally inexpensive. We evaluate our procedure on three image-to-image regression tasks: quantitative phase microscopy, accelerated magnetic resonance imaging, and super-resolution transmission electron microscopy of a Drosophila melanogaster brain.

==> Image-to-Image Regression with Distribution-Free Uncertainty Quantification and Applications in Imaging/algorithms/algo-explanatory.tex <==
\begin{algorithm}[t]
\caption{Generating Image-Valued RCPS}
\label{alg:explanatory}

\begin{algorithmic}[1]

\State Train model that outputs point prediction $\hat{f}$ and heuristic lower and upper interval lengths $\tilde{l}$ and $\tilde{u}$.
\State Compute the calibrated parameter $\hat{\lambda}$ using the calibration data and Algorithm~\ref{alg:rcps-cal}.
\State Construct $\T$ as in~\eqref{eq:nested-sets}.
\State For a new image $X$, output the risk-controlling prediction set $\T(X)$.

\end{algorithmic}

\end{algorithm}

==> Image-to-Image Regression with Distribution-Free Uncertainty Quantification and Applications in Imaging/algorithms/algo-rcps-cal.tex <==
\begin{algorithm}[b]
\caption{Pseudocode for computing $\hat{\lambda}$}
\label{alg:rcps-cal}

\textbf{Input:} Calibration data, $(X_i,Y_i)$, $i = 1, \ldots, n$; risk level $\alpha$; error rate $\delta$; underlying predictor $\hat{f}$; heuristic lower and upper interval lengths $\tilde{l}$ and $\tilde{u}$; maximum value $\lambda_{\rm max}$; step size $d\lambda > 0$.

\textbf{Output:} Parameter $\hat{\lambda}$ for computing RCPS.

\begin{algorithmic}[1]

\State $\lambda \gets \lambda_{\rm max}$
\State $r \gets 1$

\While{$r \leq \alpha$}
    \State $\lambda \gets \lambda - d\lambda$
    \For{$i=1,...,n$}  
        \State $L_i \gets L\big(\mathcal{T}_{\lambda}(X_i),Y_i\big)$
    \EndFor
    \State $r \gets \frac{1}{n}\sum\limits_{i=1}^n L_i + \sqrt{\frac{1}{2n}\log \frac{1}{\delta}}$ \Comment{Can replace with any valid upper-confidence bound on the risk.}
\EndWhile

\State $\hat{\lambda} \gets \lambda + d\lambda$ \Comment{Backtrack by one because we overshot.}
\end{algorithmic}

\end{algorithm}
